"STILL AROUND": Experiences and Survival Strategies of Veteran Women Software Developers

The intersection of ageism and sexism can create a hostile environment for veteran software developers belonging to marginalized genders. In this study, we conducted 14 interviews to examine the experiences of people at this intersection, primarily women, in order to discover the strategies they employed in order to successfully remain in the field. We identified 283 codes, which fell into three main categories: Strategies, Experiences, and Perception. Several strategies we identified, such as (Deliberately) Not Trying to Look Younger, were not previously described in the software engineering literature. We found that, in some companies, older women developers are recognized as having particular value, further strengthening the known benefits of diversity in the workforce. Based on the experiences and strategies, we suggest organizations employing software developers to consider the benefits of hiring veteran women software developers. For example, companies can draw upon the life experiences of older women developers in order to better understand the needs of customers from a similar demographic. While we recognize that many of the strategies employed by our study participants are a response to systemic issues, we still consider that, in the short-term, there is benefit in describing these strategies for developers who are experiencing such issues today.

==> interviewGuide.tex <==
\section{Interview script}\label{Appendix:Interview}
\as{Convert this to a table? Integrate in the main body of the paper?} \ab{I think it is too long and fits as an appendix.}
\begin{enumerate}
    \item \textbf{Demographic} \\
\textbf{Because of the GDPR we cannot connect the screening survey to your answers in this interview. So I am quickly going to repeat some of the questions asked in there, if you are OK with this?}
\begin{itemize}
\item What is you gender (identity)? 
\item What is your age or age range? Which ever is most comfortable
\item Are you currently working in software development?  
\end{itemize}
$[$ follow-up if they are working in the industry $]$
\begin{itemize}
\item For approximately how long have you worked in software development? 
\end{itemize}
$[$follow-up if they are not working in the industry$]$ 
\begin{itemize}
\item Approximately when did you leave?
\item For approximately how long did you work in software development?
\end{itemize}
\item \textbf{View of the industry}
\begin{itemize}
\item Can you please tell me about the positive experiences you had working in IT?
\item Can you please tell me about the negative experiences you had working in IT?
\item Why do you think you face these challenges ?
\end{itemize}

\item \textbf{View of the industry (age \& gender)}
\begin{itemize}
\item Do you feel that your gender or age influences your experience in IT?
\item Do you think the atmosphere at your work has a role to play in your experiences/not have your gender or age influence your experiences?
\item How have you dealt with these challenges?
\item Do you think you feel like you were assigned different tasks than your younger or your differently gendered colleagues throughout your career?
\end{itemize}

\item \textbf{Feeling undervalued}
\begin{itemize}
\item How do you feel your work has been valued in your career?
\end{itemize}
$[$Follow-up if undervalued$]$ 
\begin{itemize}
\item Could you tell me about situations you felt like that?
\item How did you react in those situations?
\item How long ago did this happen?
\item If significantly younger than now] How do you think you would respond to a
similar situation now?
\end{itemize}

\item \textbf{Feeling like leaving the field}
$[$ask if they left the field
\begin{itemize}
\item You mentioned you left the field, could you tell me why?
\end{itemize}
$[$if they left before retirement age$]$ 
\begin{itemize}
\item Do you think your gender or age played a role in the decision to leave software development before reaching the retirement age?
\end{itemize}
$[$Follow-up if undervalued$]$ 
\begin{itemize}
\item Do you think the feeling of being undervalued might have played a role in you leaving? 
\end{itemize}
$[$Ask If they are currently in the field$]$ 
\begin{itemize}
\item Did you ever feel like leaving IT? If so, what prompted those feelings?
\item Do you think your gender or age played a role in this feeling?
\end{itemize}
$[$Follow-up if undervalued$]$ 
\begin{itemize}
\item Do you think the feeling of being undervalued might have played a role in that feeling?
\end{itemize}
$[$Follow-up if undervalued$]$ 
\begin{itemize}
\item Could you tell me why you made the switch?
\item Did your age or gender play a role in the switch?
\item Do you think the feeling of being undervalued might have played a role in that feeling?
\end{itemize}

\item Gender and age-specific strategies
\begin{itemize}
\item Have you or those around you, adopted strategies or techniques in your working life, that you think younger colleagues or differently gendered colleagues do not need to adopt?
\begin{itemize}
\item (ask for specific aspect if they only focus on one of them)
\end{itemize}
For all or these strategies and techniques, can you tell me:
\item How old were you, approximately, when you adopted them?
\item What were your goals in adopting these strategies?
\item What do you think the benefits were of these strategies?
\item What do you think the disadvantages were of these strategies?
\item Did you continue using these strategies? If not, what led you to stop using it?
\end{itemize}

\item Existing literature
\begin{itemize}
\item The following strategies have been reported as being used by women in
male-dominated industries.
Ignoring situations, being more work oriented than family oriented, dressing
differently (i.e more feminine, less feminine, make-up) and being more passive in groups.
Do any of them seem familiar to you? Have you done any of these yourself, or
observed others doing them?
\item Research has found age-related strategies, changing appearance to look
younger (i.e dying hair, make-up), change behaviours (i.e vocabulary). Have you
noticed anyone using these strategies or similar ones?
\end{itemize}

\end{enumerate}

==> tab-participants-concise.tex <==
%\begin{table}
%\centering
%    \caption{Study Participants}
%    \label{tab:participants}
    %{\renewcommand{\arraystretch}{2}%
%    \begin{tabular}{l@{ }l@{ }l@{ }l@{ }l}
%    \toprule

%    \textbf{Pseudonym}& \textbf{Age}& \textbf{Experience}& \textbf{Gender}& \textbf{Status} \tabularnewline
%    \midrule
    
%    Alex & 55-59& 25-29& woman& active\tabularnewline
 %   Billie & 50-54& 18-24& woman& active\tabularnewline
 %   Bobbie&  60$+$& 25-29& woman& active\tabularnewline
%    Charlie & 40-44& 18-24& woman& active\tabularnewline
 %   Dani & 60$+$& 45$+$& woman& active\tabularnewline
  %  Emery & 50-54& 18-24& woman& active\tabularnewline
    % Erin &  60$+$& 45$+$& woman& active\tabularnewline % Same as Dani
%    Jackie & 60$+$& 40-44& woman& active\tabularnewline
 %   Jaime & 50-54& 25-29& woman& active\tabularnewline
 %   Robin & 45-49& 18-24& woman& active\tabularnewline
 %   Sam & 40-44& 18-24& woman& active\tabularnewline
 %   Stevie & 60$+$& 40-44& woman& active\tabularnewline
  %  \midrule
  %  Elliot & 50-54& 18-24& woman& left\tabularnewline
  %  Noah & 40-44& 18-24& non-binary& returned\tabularnewline
  %  Riley & 35-39& $<$18& woman& active\tabularnewline  
   % \bottomrule
    %
%    \end{tabular}%}
%
%
%\end{table}

\begin{table}
\centering
    \caption{Study Participants}
    \label{tab:participants}
    %{\renewcommand{\arraystretch}{2}%
    \begin{tabular}{l@{ }l@{ }l@{ }l@{ }l|l@{ }l@{ }l@{ }l@{ }l}
    \toprule

    \textbf{Pseud}& \textbf{Age}& \textbf{Exp}& \textbf{Gender}& \textbf{Status} & \textbf{Pseud}& \textbf{Age}& \textbf{Exp}& \textbf{Gender}& \textbf{Status} \tabularnewline
    \midrule
    
    Alex & 55-59& 25-29& woman& active & Jackie & 60$+$& 40-44& woman& active\tabularnewline
    Billie & 50-54& 18-24& woman& active &Jaime & 50-54& 25-29& woman& active\tabularnewline
    Bobbie&  60$+$& 25-29& woman& active & \emph{Noah} & 40-44& 18-24& non-bin& returned\tabularnewline
    Charlie & 40-44& 18-24& woman& active&\emph{Riley} & 35-39& $<$18& woman& active\tabularnewline
    Dani & 60$+$& 45$+$& woman& active & Robin & 45-49& 18-24& woman& active\tabularnewline
    \emph{Elliot} & 50-54& 18-24& woman& left&Sam & 40-44& 18-24& woman& active\tabularnewline
    Emery & 50-54& 18-24& woman& active&Stevie & 60$+$& 40-44& woman& active\tabularnewline
    % Erin &  60$+$& 45$+$& woman& active\tabularnewline % Same as Dani   
    \bottomrule
    
    \end{tabular}%}


\end{table}


